FPGAN-Control: A Controllable Fingerprint Generator for Training with Synthetic Data

Training fingerprint recognition models using synthetic data has recently gained increased attention in the biometric community as it alleviates the dependency on sensitive personal data. Existing approaches for fingerprint generation are limited in their ability to generate diverse impressions of the same finger, a key property for providing effective data for training recognition models. To address this gap, we present FPGAN-Control, an identity preserving image generation framework which enables control over the fingerprint's image appearance (e.g., fingerprint type, acquisition device, pressure level) of generated fingerprints. We introduce a novel appearance loss that encourages disentanglement between the fingerprint's identity and appearance properties. In our experiments, we used the publicly available NIST SD302 (N2N) dataset for training the FPGAN-Control model. We demonstrate the merits of FPGAN-Control, both quantitatively and qualitatively, in terms of identity preservation level, degree of appearance control, and low synthetic-to-real domain gap. Finally, training recognition models using only synthetic datasets generated by FPGAN-Control lead to recognition accuracies that are on par or even surpass models trained using real data. To the best of our knowledge, this is the first work to demonstrate this.

==> tables/table_10K_synth.tex <==
\begin{table*}[h]
    \centering
    %\vskip 0.15in
    \small
    
    \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
    %\renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l | C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth}}
        \toprule
        \textbf{Training dataset}    & \textbf{Res18}         & \textbf{Res34}          & \textbf{Res50}   & \textbf{Res101}  & \textbf{Mob-050} & \textbf{Mob-100} & \textbf{Eff-s} \\ %\hline
        \midrule
        Real data         & $90.54$        & $89.72$        & $92.00$ & $93.69$        & $93.74$ & $94.22$ & $93.69$ \\
        \midrule
        StyleGAN2         & $12.57$        & $5.46$         & $5.86$  & $4.07$         & $38.16$ & $19.36$ & $16.18$    \\
        PrintsGAN         & $61.30$        & $56.30$        & $62.17$ & $67.20$        & $69.88$ & $76.58$ & $68.05$    \\ 
        FPGC-0           & $80.23$        & $75.17$        & $80.39$ & $88.57$        & $88.55$ & $89.75$ & $80.01$    \\ 
        FPGC-0.25        &  $80.42$         & $78.27$          & $81.48$   &  $90.29$         & $87.68$ & $88.78$ & $80.39$    \\
        FPGC-0.5         &  $81.37$         & $79.14$          & $82.88$   &  $89.38$         & $87.46$ & $89.52$ & $81.83$    \\
        FPGC-1           & $85.58$        & $81.64$          & $82.82$   &  $89.81$         & $\textbf{89.25}$ & $\textbf{89.76}$ & $82.95$    \\
        FPGC-5           &  $82.02$         & $79.27$          & $81.02$   &  $82.20$         & $87.25$ & $87.78$ & $79.87$                    \\
        FPGC-20          & $\textbf{85.90}$ & $\textbf{84.36}$ & $\textbf{84.38}$ & $\textbf{91.07}$ & $88.57$ & $89.28$ & $\textbf{87.82}$   \\
        \midrule
        FPGC-0.25 + FPGC-20   & $87.20$          & $86.10$          & $\textbf{88.00}$ & $91.63$          & $\textbf{91.19}$ & $92.08$ & $89.32$  \\
        FPGC-0.5 + FPGC-20    & $87.29$          & $86.04$          & $87.25$          & $\textbf{92.81}$ & $91.01$ & $\textbf{92.12}$ & $90.13$  \\
        FPGC-1 + FPGC-20       & $87.65$          & $\textbf{87.01}$ & $87.47$          & $92.08$          & $90.99$ & $91.64$ & $89.46$  \\
        FPGC-5 + FPGC-20       & $\textbf{87.77}$ & $86.76$          & $86.13$          & $91.12$          & $90.86$ & $91.44$ & $\textbf{90.22}$  \\
        % FPGAN (All)     & -           & \textbf{88.50} &         &         & FAILED         &         &         &   \\
        \bottomrule
    \end{tabular}
    \caption{
    % TAR@FAR0.1\% results of various recognition models trained using different synthetic datasets for xx backbones.
    \textbf{Recognition results for 10K synthetic identities.}
    TAR@FAR=0.1\% results obtained by recognition models with various backbones trained using different synthetic datasets for the case of \textbf{10K} synthetic identities. 
    % Each dataset generated by a specific FPGAN-control is denoted as FPGC-$w_{app}$ following the corresponding appearance loss weight.
    % Each dataset that was generated by a FPGAN-control model with a different $w_{app}$ is denoted by FPGC-$w_{app}$.
    The datasets that were generated by FPGAN-control are denoted by FPGC-$w_{app}$ where $w_{app}$ corresponds to the weight of the appearance loss.
    }
    \label{tab:10k_synth}

\end{table*}


% \begin{table*}[t]
%     \centering
%     %\vskip 0.15in
%     \small
    
%     \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{l c | C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth} C{0.08\textwidth}}
%         \toprule
%         Training dataset & App loss    & Res18         & Res34          & Res50   & Res101  & Mob-050 & Mob-100 & Eff-s \\ %\hline
%         \midrule
%         Real data       &             & $90.54$        & $89.72$        & $92.00$ & $93.69$        & $93.74$ & $94.22$ & $93.69$ \\
%         \midrule
%         StyleGAN2       &             & $12.57$        & $5.46$         & $5.86$  & $4.07$         & $38.16$ & $19.36$ & $16.18$    \\
%         PrintsGAN       &             & $61.30$        & $56.30$        & $62.17$ & $67.20$        & $69.88$ & $76.58$ & $68.05$    \\ 
%         FPGAN-0         & $0$         & $80.23$        & $75.17$        & $80.39$ & $88.57$        & $88.55$ & $89.75$ & $80.01$    \\ 
%         FPGAN-0.25      & $0.25$      &  80.42         & 78.27          & 81.48   &  90.29         & $87.68$ & $88.78$ & $80.39$    \\
%         FPGAN-0.5       & $0.50$      &  81.37         & 79.14          & 82.88   &  89.38         & $87.46$ & $89.52$ & $81.83$    \\
%         FPGAN-1         & $1$         & $85.58$        & 81.64          & 82.82   &  89.81         & $\textbf{89.25}$ & $\textbf{89.76}$ & $82.95$    \\
%         FPGAN-5         & $5$         &  82.02         & 79.27          & 81.02   &  82.20         & $87.25$ & $87.78$ & $79.87$                    \\
%         FPGAN-20        & $20$        & \textbf{85.90} & \textbf{84.36} & \textbf{84.38} & \textbf{91.07} & $88.57$ & $89.28$ & $\textbf{87.82}$   \\
%         \midrule
%         FPGAN-(0.25,20) & $(0.25,20)$ & 87.20          & 86.10          & \textbf{88.00} & 91.63          & $\textbf{91.19}$ & $92.08$ & $89.32$  \\
%         FPGAN-(0.5,20)  & $(0.5,20)$  & 87.29          & 86.04          & 87.25          & \textbf{92.81} & $91.01$ & $\textbf{92.12}$ & $90.13$  \\
%         FPGAN-(1,20)    & $(1,20)$    & 87.65          & \textbf{87.01} & 87.47          & 92.08          & $90.99$ & $91.64$ & $89.46$  \\
%         FPGAN-(5,20)    & $(5,20)$    & \textbf{87.77} & 86.76          & 86.13          & 91.12          & $90.86$ & $91.44$ & $\textbf{90.22}$  \\
%         % FPGAN (All)     & -           & \textbf{88.50} &         &         & FAILED         &         &         &   \\
%         \bottomrule
%     \end{tabular}
%     \caption{10K synth 0 real.}
%     \label{tab:10k_synth}

% \end{table*}


%Ours5     & $1.0$ & $5.00$  &         &         &         &         & $86.06$ & $83.65$ &     \\
        %Ours6     & $2.0$ & $10.00$ &         &         &         &         & $83.04$ & $82.32$ &     \\

==> tables/table_fid.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l c c c c c c}
    \toprule
    $w_{app}$ \quad\quad\quad   & $0$    & $0.25$ & $0.5$ & $1$ & $5$ & $20$ \\
    \midrule
    FID$\downarrow$ & $4.74$ & $4.72$ & $5.56$ & $4.73$ & $5.04$ & $5.61$ \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{FID scores of FPGAN-Control models trained with different $w_{app}$ values.}}
    \label{tab:fid}
\end{table}


% \midrule
%     $0.00$ & $0.063$\tiny{$\pm0.06$} & $0.026$\tiny{$\pm0.04$} & $0.055$\tiny{$\pm0.04$} & $4.74$ \\
%     % $0.50$ & $0.061$\tiny{$\pm0.05$} & $0.032$\tiny{$\pm0.04$} & $0.039$\tiny{$\pm0.03$} & $5.78$ \\
%     $1.00$ & $0.106$\tiny{$\pm0.11$} & $0.043$\tiny{$\pm0.04$} & $0.025$\tiny{$\pm0.02$} & $4.73$ \\
%     $5.00$ & $0.206$\tiny{$\pm0.10$} & $0.051$\tiny{$\pm0.05$} & $0.008$\tiny{$\pm0.00$} & $5.04$ \\
%     $20.0$ & $0.254$\tiny{$\pm0.11$} & $0.057$\tiny{$\pm0.05$} & $0.002$\tiny{$\pm0.00$} & $5.61$ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Distribution change vs. appearance loss.}
%     \label{tab:appearance_change}

==> tables/table_quantative.tex <==
\begin{table}[t]
    \centering
    %\vskip 0.15in
    \small
    \begin{tabular}{l | c c c c}
    \toprule
    % ID \newline loss & Appearance \newline loss & ID \newline preservation$\downarrow$ & Appearance \newline variation$\uparrow$ & Appearance \newline preservation$\downarrow$ & FID$\downarrow$ \\
    
    App. \quad\quad\quad & ID dist & App. dist & App. dist & FID$\downarrow$ \\
    loss & same ID & same ID & same App. & \\
    \midrule
    Real data & $0.375$\tiny{$\pm0.19$} & $0.058$\tiny{$\pm0.05$} & N/A &    \\
    \midrule
    $0.00$ & $0.063$\tiny{$\pm0.06$}    & $0.026$\tiny{$\pm0.04$} & $0.055$\tiny{$\pm0.04$} & $4.74$ \\
    % $0.50$ & $0.061$\tiny{$\pm0.05$} & $0.032$\tiny{$\pm0.04$} & $0.039$\tiny{$\pm0.03$} & $5.78$ \\
    $1.00$ & $0.122$\tiny{$\pm0.08$}     & $0.043$\tiny{$\pm0.04$} & $0.025$\tiny{$\pm0.02$} & $4.73$ \\
    $5.00$ & $0.229$\tiny{$\pm0.11$}     & $0.051$\tiny{$\pm0.05$} & $0.008$\tiny{$\pm0.00$} & $5.04$ \\
    $20.0$ & $0.283$\tiny{$\pm0.11$}     & $0.057$\tiny{$\pm0.05$} & $0.002$\tiny{$\pm0.00$} & $5.61$ \\
    \bottomrule
    \end{tabular}
    \caption{Distribution change vs. appearance loss.}
    \label{tab:appearance_change}
\end{table}


% \midrule
%     $0.00$ & $0.063$\tiny{$\pm0.06$} & $0.026$\tiny{$\pm0.04$} & $0.055$\tiny{$\pm0.04$} & $4.74$ \\
%     % $0.50$ & $0.061$\tiny{$\pm0.05$} & $0.032$\tiny{$\pm0.04$} & $0.039$\tiny{$\pm0.03$} & $5.78$ \\
%     $1.00$ & $0.106$\tiny{$\pm0.11$} & $0.043$\tiny{$\pm0.04$} & $0.025$\tiny{$\pm0.02$} & $4.73$ \\
%     $5.00$ & $0.206$\tiny{$\pm0.10$} & $0.051$\tiny{$\pm0.05$} & $0.008$\tiny{$\pm0.00$} & $5.04$ \\
%     $20.0$ & $0.254$\tiny{$\pm0.11$} & $0.057$\tiny{$\pm0.05$} & $0.002$\tiny{$\pm0.00$} & $5.61$ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Distribution change vs. appearance loss.}
%     \label{tab:appearance_change}
